Learning to Execute

Recurrent Neural Networks (RNNs) with Long Short-Term Memory units (LSTM) are widely used because they are expressive and are easy to train. Our interest lies in empirically evaluating the expressiveness and the learnability of LSTMs in the sequence-to-sequence regime by training them to evaluate short computer programs, a domain that has traditionally been seen as too complex for neural networks. We consider a simple class of programs that can be evaluated with a single left-to-right pass using constant memory. Our main result is that LSTMs can learn to map the character-level representations of such programs to their correct outputs. Notably, it was necessary to use curriculum learning, and while conventional curriculum learning proved ineffective, we developed a new variant of curriculum learning that improved our networks' performance in all experimental conditions. The improved curriculum had a dramatic impact on an addition problem, making it possible to train an LSTM to add two 9-digit numbers with 99% accuracy.

==> Makefile <==
PARTS=algebra.tex

all: clean algebra.pdf 

algebra.pdf: $(PARTS) bibliography.bib 
	pdflatex -shell-escape algebra.tex
	pdflatex -shell-escape algebra.tex
	pdflatex -shell-escape algebra.tex
	bibtex algebra
	bibtex algebra
	bibtex algebra
	pdflatex -shell-escape algebra.tex
	pdflatex -shell-escape algebra.tex

clean:
	rm -f *.log *.blg *.aux *.bbl *.4tc *.xref *.tmp *.dvi *.hd *.idx *.out *.toc *.drv *.ins *.pdf
	rm -rf ~*
	rm -rf *.tmp
	rm -rf *.4om
	rm -rf *~

tar:
	find . -type f | egrep -v '\.git|\.log|\.swp' | xargs tar zcvf ../algebra.tar.gz

